Automated Identification of Vulnerable Devices in Networks using Traffic Data and Deep Learning

Many IoT devices are vulnerable to attacks due to flawed security designs and lacking mechanisms for firmware updates or patches to eliminate the security vulnerabilities. Device-type identification combined with data from vulnerability databases can pinpoint vulnerable IoT devices in a network and can be used to constrain the communications of vulnerable devices for preventing damage. In this contribution, we present and evaluate two deep learning approaches to the reliable IoT device-type identification, namely a recurrent and a convolutional network architecture. Both deep learning approaches show accuracies of 97% and 98%, respectively, and thereby outperform an up-to-date IoT device-type identification approach using hand-crafted fingerprint features obtaining an accuracy of 82%. The runtime performance for the IoT identification of both deep learning approaches outperforms the hand-crafted approach by three magnitudes. Finally, importance metrics explain the results of both deep learning approaches in terms of the utilization of the analyzed traffic data flow.

==> abstractVS.tex <==
\begin{abstract}

Many IoT devices are vulnerable to hackers due to flawed security designs and lacking mechanisms for firmware updates or patches to eliminate the security vulnerabilities.
%
Device-type identification combined with data from vulnerability databases can pinpoint vulnerable IoT devices in a network and can be used to constrain the communications of vulnerable devices for preventing damage. 
%
In this contribution, we present and evaluate two deep learning approaches to the reliable IoT device-type identification, namely a recurrent and a convolutional network architecture. Both approaches show accuracies of 97\% and 98\%, respectively, and thereby outperform an up-to-date IoT device-type identification approach using hand-crafted fingerprint features obtaining an accuracy of 82\%.

\end{abstract}

==> chapters/abstract.tex <==
\begin{quotation}
\section*{\centering \begin{normalsize}Abstract\end{normalsize}}
In our increasingly connected world IoT devices play a crucial role. 
IoT devices do not only collect, process and transmit sensitive data, they also control more and more functionalities and features in our homes. 
From intelligent heating to voice-controlled speakers and smart cameras, these devices are already present in every area of our lives. 
IoT devices can be found in almost every household today, but this is accompanied by a high-security risk. 
One possible solution would require the precise identification of IoT devices. 
But identification of IoT devices in network traffic without prior knowledge of the devices present in the network is a demanding task.

In this study we compare different algorithms of machine learning on their ability to classify IoT traffic data. 
Especially, we considered how handcrafted features behave in comparison to automatically deep learned features. 
Firstly handcrafted features using three different machine learning methods are classified. 
Then deep learning is used to automatically learned representative features from raw traffic data, afterwards both futures extraction methods are compared. 
It is also investigated how different data granularities affect the accuracy of the algorithms. 
We achieved higher accuracies when features are automatically learned, rather than manually selected.

\end{quotation}
\clearpage

==> chapters/deviceTypes.tex <==
\begin{table}[H]
\centering
\begin{tabular}{lll}
\toprule
Identifier & Device Model & Connectivity \\
\midrule
Aria & Fitbit Aria WiFi-enabled scale & WiFi\\
HomeMaticPlug & Homematic pluggable switch HMIP-PS & ZigBee\\
Withings & Withings Wireless Scale WS-30 & WiFi\\
MAXGateway & MAX! Cube LAN Gateway for MAX! Home automation sensors & Ethernet/Others\\
HueBridge & Philips Hue Bridge model 3241312018 & ZigBee/Ethernet\\
HueSwitch & Philips Hue Light Switch PTM 215Z & ZigBee\\
EdnetGateway & Ednet.living Starter kit power Gateway & WiFi/Other\\
EdnetCam & Ednet Wireless indoor IP camera Cube & ZigBee/Ethernet\\
EdimaxCam & Edimax IC-3115W Smart HD WiFi Network Camera & ZigBee/Ethernet\\
Lightify & Osram Lightify Gateway & WiFi/Ethernet\\
WeMoInsightSwitch & WeMo Insight Switch model F7C029de & WiFi\\
WeMoLink & WeMo Link Lighting Bridge model F7C031vf  & WiFi/Ethernet\\
WeMoSwitch & WeMo Switch model F7C027de  & WiFi\\
D-LinkHomeHub & D-Link Connected Home Hub DCH-G020 & WiFi/Ethernet/Z-Wave\\
D-LinkDoorSensor & D-Link Door Window sensor & Z-Wave\\
D-LinkDayCam & D-Link WiFi Day Camera DCS-930L  & WiFi/Ethernet\\
D-LinkCam & D-Link HD IP Camera DCH-935L  & WiFi\\
D-LinkSwitch & D-Link Smart plug DSP-W215  & WiFi\\
D-LinkWaterSensor & D-Link Water sensor DCH-S160  & WiFi\\
D-LinkSiren & D-Link Siren DCH-S220  & WiFi\\
D-LinkSensor & D-Link WiFi Motion sensor DCH-S150  & WiFi\\
TP-LinkPlugHS110 & TP-Link WiFi Smart plug HS110  & WiFi\\
TP-LinkPlugHS100 & TP-Link WiFi Smart plug HS100  & WiFi\\
EdimaxPlug1101W & Edimax SP-1101W Smart Plug Switch  & WiFi\\
EdimaxPlug2101W & Edimax SP-2101W Smart Plug Switch  & WiFi\\
SmarterCoffee & Smarter SmarterCoffee coffee machine SMC10-EU  & WiFi\\
iKettle2 & Smarter iKettle 2.0 water kettle SMK20-EU  & WiFi\\
\bottomrule
\end{tabular}
  \caption{IoT device types of the IoT SENTINEL dataset and their supported connectivity.}
  \label{tab:SentinelDevices}
\end{table}
